Gridding and Parameter Expansion for Scalable Latent Gaussian Models of Spatial Multivariate Data

Scalable spatial GPs for massive datasets can be built via sparse Directed Acyclic Graphs (DAGs) where a small number of directed edges is sufficient to flexibly characterize spatial dependence. The DAG can be used to devise fast algorithms for posterior sampling of the latent process, but these may exhibit pathological behavior in estimating covariance parameters. In this article, we introduce gridding and parameter expansion methods to improve the practical performance of MCMC algorithms in terms of effective sample size per unit time (ESS/s). Gridding is a model-based strategy that reduces the number of expensive operations necessary during MCMC on irregularly spaced data. Parameter expansion reduces dependence in posterior samples in spatial regression for high resolution data. These two strategies lead to computational gains in the big data settings on which we focus. We consider popular constructions of univariate spatial processes based on Mat\'ern covariance functions and multivariate coregionalization models for Gaussian outcomes in extensive analyses of synthetic datasets comparing with alternative methods. We demonstrate effectiveness of our proposed methods in a forestry application using remotely sensed data from NASA's Goddard LiDAR, Hyper-Spectral, and Thermal imager (G-LiHT).

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -pdf \"$_[0]\"" );
    }
}

==> noncentered_param_tikz.tex <==
% draw dag
\usepackage{tikz}
\usetikzlibrary{bayesnet}

\begin{comment}
\usetikzlibrary{shapes,decorations,arrows,calc,arrows.meta,fit,positioning}
\tikzset{
    -Latex,auto,node distance =1 cm and 1 cm,semithick,
    state/.style ={ellipse, draw, minimum width = 0.7 cm},
    point/.style = {circle, draw, inner sep=0.04cm,fill,node contents={}},
    bidirected/.style={Latex-Latex,dashed},
    el/.style = {inner sep=2pt, align=left, sloped}
}
\end{comment}

\begin{document}

\begin{tikzpicture}
  % Define nodes
  \node[obs] (y) {$\by$};
  \node[latent, left=of y, yshift=.5cm] (w) {$\bw$};
  \node[const, above=of w] (empty) { };
  \node[latent, left=of w]  (theta) {$\btheta$};
  \node[latent, left=of y, yshift=-.5cm] (t) {$\bbeta, \btau$};
  % Connect the nodes
  \edge {w} {y} ; %
  \edge {t} {y} ; %
  \edge {theta} {w} ; %
\end{tikzpicture} 
  \caption{Centered parametrization}
  \label{fig:param:centered}
\end{subfigure}
\begin{subfigure}{.5\textwidth}
  \centering
  % include second image
\begin{tikzpicture}
  % Define nodes
  \node[obs]                               (y) {$\by$};
  \node[latent, left=of y, yshift=1cm] (lam) {$\bLambda$};
  \node[latent, left=of y] (w) {$\bomega$};
  \node[latent, left=of w]  (phi) {$\bvarphi$};
  \node[latent, left=of y, yshift=-1cm] (t) {$\bbeta, \btau$};
  % Connect the nodes
  \edge {lam} {y} ; %
  \edge {w} {y} ; %
  \edge {t} {y} ; %
  \edge {phi} {w} ; %
\end{tikzpicture}

\end{document}

==> preamble.tex <==

%% This document created by Scientific Word (R) Version 3.5
%\usepackage{psfig}

\makeatletter
\setlength{\@fptop}{0pt}
\makeatother

%\addtolength{\oddsidemargin}{-.5in}%
%\addtolength{\evensidemargin}{-.5in}%
%\addtolength{\textwidth}{1in}%
%\addtolength{\textheight}{1.3in}%
%\addtolength{\topmargin}{-.8in}%


\RequirePackage{etoolbox}
\csdef{input@path}{%
	%{sty/}% cls, sty files
	{img/}% eps files
}%

% packages
%\usepackage{hyperref} %This removes the boxes around the links
\usepackage{xr-hyper}
\usepackage[colorlinks,citecolor=blue,urlcolor=blue,filecolor=blue,backref=page]{hyperref}
\usepackage{gensymb}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsbsy}
\usepackage{amsthm}
\usepackage{mathtools}
\usepackage{mathbbol}
\usepackage{mathrsfs}
\usepackage{bbm} 
\usepackage{graphicx,psfrag,epsf}
\usepackage{enumerate}
\usepackage{natbib}
\usepackage{url} 
\usepackage{float}
\usepackage[skip=5pt]{caption}
\usepackage{subcaption}
\usepackage[normalem]{ulem}
\usepackage{comment}
\usepackage{hhline}
\usepackage{afterpage}
\usepackage{multirow}
\usepackage{adjustbox}
\usepackage{textcomp}
\usepackage{rotating}
\usepackage{tabularx}
\usepackage{xspace}

\usepackage{color,colortbl,soul}
\usepackage[dvipsnames]{xcolor}
\usepackage{blkarray}

\usepackage[boxed, vlined]{algorithm2e}
\usepackage[T1]{fontenc}
\usepackage{arydshln}
\usepackage{scalerel,stackengine}
%\usepackage[hmargin=1.0in,vmargin=1.0in]{geometry}

\usepackage{algorithmicx}
\usepackage{algpseudocode}

\usepackage{lipsum}
\usepackage{listings}
\usepackage{cancel}

\lstset{
    language=R,
    basicstyle=\tiny
    %basicstyle=\ttfamily
}

% algorithm options
\SetAlCapSkip{.5em}

% colors
\definecolor{Gray}{gray}{0.9}


\allowdisplaybreaks

% commands

\makeatletter
\renewcommand*\env@matrix[1][*\c@MaxMatrixCols c]{%
	\hskip -\arraycolsep
	\let\@ifnextchar\new@ifnextchar
	\array{#1}}
\makeatother

\newcommand*{\arXiv}[1]{\small\texttt{\href{http://arxiv.org/abs/#1}{arXiv:#1}}}
\newcommand*{\doib}[1]{\small\texttt{\href{http://dx.doi.org/#1}{doi:#1}}}
%\RequirePackage{doi}

\newcommand{\iidsim}{\overset{iid}{\sim}} % iid 

\newcommand{\highlight}[1]{%
	\colorbox{yellow!50}{$\displaystyle#1$}}

\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}

\newcommand{\matrow}[2]{{#1}\texttt{[{#2},:]}}

\newcommand{\given}{\,|\,}


\stackMath
\newcommand\reallywidehat[1]{%
	\savestack{\tmpbox}{\stretchto{%
			\scaleto{%
				\scalerel*[\widthof{\ensuremath{#1}}]{\kern-.6pt\bigwedge\kern-.6pt}%
				{\rule[-\textheight/2]{1ex}{\textheight}}%WIDTH-LIMITED BIG WEDGE
			}{\textheight}% 
		}{0.5ex}}%
	\stackon[1pt]{#1}{\tmpbox}%
}

\theoremstyle{definition}
\newtheorem{assumption}{Assumption}[section]
\newtheorem{definition}{Definition}[section]
\newtheorem{lemma}{Lemma}[section]
\newtheorem{proposition}{Proposition}[section]
\newtheorem{corollary}{Corollary}[section]

\makeatletter
\newcommand*{\addFileDependency}[1]{% argument=file name and extension
  \typeout{(#1)}
  \@addtofilelist{#1}
  \IfFileExists{#1}{}{\typeout{No file #1.}}
}
\makeatother

\newcommand*{\myexternaldocument}[1]{%
    \externaldocument{#1}%
    \addFileDependency{#1.tex}%
    \addFileDependency{#1.aux}%
}


\def\mathcolor#1#{\@mathcolor{#1}}
\def\@mathcolor#1#2#3{%
	\protect\leavevmode
	\begingroup
	\color#1{#2}#3%
	\endgroup
}
% draw dag
\usepackage{tikz}
\usetikzlibrary{bayesnet}



% symbols
\renewcommand{\tilde}[1]{\widetilde{#1}}

\newcommand{\textalt}[1]{\quad\text{#1}\quad}
\newcommand{\sigmasq}{\sigma^2}

\newcommand{\is}[1]{\text{\usefont{U}{bbm}{m}{n}#1}} % from mathbbm.sty
\newcommand{\bml}{b}
\newcommand{\bolds}[1]{\boldsymbol{#1}}
%\newcommand{\bm}[1]{\mathbf{#1}}

% boldcal
\newcommand{\bcA}{\bolds{{\cal A}}}
\newcommand{\bcH}{\bolds{{\cal H}}}
\newcommand{\bcR}{\bolds{{\cal R}}}
\newcommand{\bcZ}{\bolds{{\cal Z}}}

% cal
\newcommand{\calA}{{\cal A}}
\newcommand{\calD}{{\cal D}}
\newcommand{\calG}{{\cal G}}
\newcommand{\calI}{{\cal I}}
\newcommand{\calK}{{\cal K}}
\newcommand{\calL}{{\cal L}}
\newcommand{\calM}{{\cal M}}
\newcommand{\calP}{{\cal P}}
\newcommand{\calQ}{{\cal Q}}
\newcommand{\calS}{{\cal S}}
\newcommand{\calT}{{\cal T}}
\newcommand{\calU}{{\cal U}}
\newcommand{\calV}{{\cal V}}
\newcommand{\calX}{{\cal X}}

\newcommand{\Cov}{\bolds{C}}

% bold
\newcommand{\ba}{\bolds{a}}
\newcommand{\bA}{\bolds{A}}
\newcommand{\bb}{\bolds{b}}
\newcommand{\bB}{\bolds{B}}
\newcommand{\bc}{\bolds{c}}
\newcommand{\bC}{\bolds{C}}
\newcommand{\bd}{\bolds{d}}
\newcommand{\bD}{\bolds{D}}
\newcommand{\be}{\bolds{e}}
\newcommand{\bE}{\bolds{E}}
\newcommand{\bbf}{\bolds{f}}
\newcommand{\bF}{\bolds{F}}
\newcommand{\bg}{\bolds{g}}
\newcommand{\bG}{\bolds{G}}
\newcommand{\bh}{\bolds{h}}
\newcommand{\bH}{\bolds{H}}
\newcommand{\bi}{\bolds{i}}
\newcommand{\bI}{\bolds{I}}
\newcommand{\bJ}{\bolds{J}}
\newcommand{\bk}{\bolds{k}}
\newcommand{\bK}{\bolds{K}}
\newcommand{\bl}{\bolds{\ell}}
\newcommand{\bL}{\bolds{L}}
\newcommand{\bm}{\bolds{m}}
\newcommand{\bM}{\bolds{M}}
\newcommand{\bn}{\bolds{N}}
\newcommand{\bN}{\bolds{N}}
\newcommand{\bO}{\bolds{O}}
\newcommand{\bp}{\bolds{p}}
\newcommand{\bP}{\bolds{P}}
\newcommand{\bQ}{\bolds{Q}}
\newcommand{\br}{\bolds{r}}
\newcommand{\bR}{\bolds{R}}
\newcommand{\bs}{\bolds{s}}
\newcommand{\bS}{\bolds{S}}
\newcommand{\bt}{\bolds{t}}
\newcommand{\bT}{\bolds{T}}
\newcommand{\bu}{\bolds{u}}
\newcommand{\bU}{\bolds{U}}
\newcommand{\bv}{\bolds{v}}
\newcommand{\bV}{\bolds{V}}
\newcommand{\bw}{\bolds{w}}
\newcommand{\bW}{\bolds{W}}
\newcommand{\bx}{\bolds{x}}
\newcommand{\bX}{\bolds{X}}
\newcommand{\by}{\bolds{y}}
\newcommand{\bY}{\bolds{Y}}
\newcommand{\bz}{\bolds{z}}
\newcommand{\bZ}{\bolds{Z}}

\newcommand{\bzero}{\mathbf{0}}

% greek
\newcommand{\bbeta}{\bolds{\beta}}
\newcommand{\btau}{\bolds{\tau}}
\newcommand{\beps}{\bolds{\varepsilon}}
\newcommand{\btheta}{\bolds{\theta}}
\newcommand{\bomega}{\bolds{\omega}}
\newcommand{\brho}{\bolds{\rho}}
\newcommand{\bphi}{\bolds{\phi}}
\newcommand{\bSigma}{\bolds{\Sigma}}
\newcommand{\bsigma}{\bolds{\sigma}}
\newcommand{\bgamma}{\bolds{\gamma}}
\newcommand{\bGamma}{\bolds{\Gamma}}
\newcommand{\bLambda}{\bolds{\Lambda}}
\newcommand{\blambda}{\bolds{\lambda}}
\newcommand{\bDelta}{\bolds{\Delta}}
\newcommand{\bPsi}{\bolds{\Psi}}
\newcommand{\bmu}{\bolds{\mu}}
\newcommand{\bnu}{\bolds{\nu}}
\newcommand{\bxi}{\bolds{\xi}}
\newcommand{\boldeta}{\bolds{\eta}}
\newcommand{\bvarphi}{\bolds{\varphi}}

% graph
\newcommand{\bwpa}[1]{\bw_{[{#1}]}}
\newcommand{\bwpaone}[1]{\bw_{[{#1}]_1}}
\newcommand{\bwpatwo}[1]{\bw_{[{#1}]_2}}
\newcommand{\Spa}[1]{\calS_{[{#1}]}}
\newcommand{\pa}[1]{\text{Pa}[{#1}]}
\newcommand{\pazero}[1]{\text{Pa}_0[{#1}]}
\newcommand{\paone}[1]{\text{Pa}_1[{#1}]}
\newcommand{\patwo}[1]{\text{Pa}_2[{#1}]}
\newcommand{\ch}[1]{\text{Ch}[{#1}]}
\newcommand{\bdiag}{\text{blockdiag}}
\newcommand{\tp}{\widetilde{p}}

\newcommand*\rot{\rotatebox{60}}




\newenvironment{smallbmat}
  {\left[\begin{smallmatrix}}
  {\end{smallmatrix}\right]}
  
\usepackage{tcolorbox}
\newtcolorbox[auto counter]{reviewcommentinside}[1][]{box align=center,
    width=0.9\textwidth,
    colframe = teal,
    colback=teal!10,
    code={\spacingset{0.9}},
    #1}
\newenvironment{reviewercomment}{%
\begin{center}
\begin{reviewcommentinside}\noindent \small 
}
{\end{reviewcommentinside}
\end{center}}

\newtcolorbox[auto counter]{importantinside}[1][]{box align=center,
    width=0.95\textwidth,
    colframe = orange,
    colback=orange!10,
    code={\spacingset{1.1}},
    #1}
\newenvironment{important}{%
\begin{center}
\begin{importantinside}\noindent 
}
{\end{importantinside}
\end{center}}



\newtcolorbox[auto counter]{reviewanswerinside}[1][]{box align=center,
    width=0.98\textwidth,
    colframe = orange!10,
    colback= orange!10,
    code={\spacingset{0.9}},
    #1}

\newenvironment{revieweranswer}{%
\begin{center}
\begin{reviewanswerinside}\noindent \footnotesize 
}
{\end{reviewanswerinside}
\end{center}}


==> tikzlibrarybayesnet.code.tex <==
% tikzlibrary.code.tex
%
% Copyright 2010-2011 by Laura Dietz
% Copyright 2012 by Jaakko Luttinen
%
% The MIT License
%
% See LICENSE file for more details.

% Load other libraries
\usetikzlibrary{shapes}
\usetikzlibrary{fit}
\usetikzlibrary{chains}
\usetikzlibrary{arrows}

% Latent node
\tikzstyle{latent} = [circle,fill=white,draw=black,inner sep=1pt,
minimum size=20pt, font=\fontsize{10}{10}\selectfont, node distance=1]
% Observed node
\tikzstyle{obs} = [latent,fill=gray!25]
% Constant node
\tikzstyle{const} = [rectangle, inner sep=0pt, node distance=1]
% Factor node
\tikzstyle{factor} = [rectangle, fill=black,minimum size=5pt, inner
sep=0pt, node distance=0.4]
% Deterministic node
\tikzstyle{det} = [latent, diamond]

% Plate node
\tikzstyle{plate} = [draw, rectangle, rounded corners, fit=#1]
% Invisible wrapper node
\tikzstyle{wrap} = [inner sep=0pt, fit=#1]
% Gate
\tikzstyle{gate} = [draw, rectangle, dashed, fit=#1]

% Caption node
\tikzstyle{caption} = [font=\footnotesize, node distance=0] %
\tikzstyle{plate caption} = [caption, node distance=0, inner sep=0pt,
below left=5pt and 0pt of #1.south east] %
\tikzstyle{factor caption} = [caption] %
\tikzstyle{every label} += [caption] %

%\pgfdeclarelayer{b}
%\pgfdeclarelayer{f}
%\pgfsetlayers{b,main,f}

% \factoredge [options] {inputs} {factors} {outputs}
\newcommand{\factoredge}[4][]{ %
  % Connect all nodes #2 to all nodes #4 via all factors #3.
  \foreach \f in {#3} { %
    \foreach \x in {#2} { %
      \path (\x) edge[-,#1] (\f) ; %
      %\draw[-,#1] (\x) edge[-] (\f) ; %
    } ;
    \foreach \y in {#4} { %
      \path (\f) edge[->, >={triangle 45}, #1] (\y) ; %
      %\draw[->,#1] (\f) -- (\y) ; %
    } ;
  } ;
}

% \edge [options] {inputs} {outputs}
\newcommand{\edge}[3][]{ %
  % Connect all nodes #2 to all nodes #3.
  \foreach \x in {#2} { %
    \foreach \y in {#3} { %
      \path (\x) edge [->, >={triangle 45}, #1] (\y) ;%
      %\draw[->,#1] (\x) -- (\y) ;%
    } ;
  } ;
}

% \factor [options] {name} {caption} {inputs} {outputs}
\newcommand{\factor}[5][]{ %
  % Draw the factor node. Use alias to allow empty names.
  \node[factor, label={[name=#2-caption]#3}, name=#2, #1,
  alias=#2-alias] {} ; %
  % Connect all inputs to outputs via this factor
  \factoredge {#4} {#2-alias} {#5} ; %
}

% \plate [options] {name} {fitlist} {caption}
\newcommand{\plate}[4][]{ %
  \node[wrap=#3] (#2-wrap) {}; %
  \node[plate caption=#2-wrap] (#2-caption) {#4}; %
  \node[plate=(#2-wrap)(#2-caption), #1] (#2) {}; %
}

% \gate [options] {name} {fitlist} {inputs}
\newcommand{\gate}[4][]{ %
  \node[gate=#3, name=#2, #1, alias=#2-alias] {}; %
  \foreach \x in {#4} { %
    \draw [-*,thick] (\x) -- (#2-alias); %
  } ;%
}

% \vgate {name} {fitlist-left} {caption-left} {fitlist-right}
% {caption-right} {inputs}
\newcommand{\vgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-left) {}; %
  \node[wrap=#4] (#1-right) {}; %
  % Draw the gate
  \node[gate=(#1-left)(#1-right)] (#1) {}; %
  % Add captions
  \node[caption, below left=of #1.north ] (#1-left-caption)
  {#3}; %
  \node[caption, below right=of #1.north ] (#1-right-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.north) -- (#1.south); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

% \hgate {name} {fitlist-top} {caption-top} {fitlist-bottom}
% {caption-bottom} {inputs}
\newcommand{\hgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-top) {}; %
  \node[wrap=#4] (#1-bottom) {}; %
  % Draw the gate
  \node[gate=(#1-top)(#1-bottom)] (#1) {}; %
  % Add captions
  \node[caption, above right=of #1.west ] (#1-top-caption)
  {#3}; %
  \node[caption, below right=of #1.west ] (#1-bottom-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.west) -- (#1.east); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

